Program Size and Temperature in Self-Assembly

Winfree's abstract Tile Assembly Model (aTAM) is a model of molecular self-assembly of DNA complexes known as tiles, which float freely in solution and attach one at a time to a growing "seed" assembly based on specific binding sites on their four sides. We show that there is a polynomial-time algorithm that, given an n x n square, finds the minimal tile system (i.e., the system with the smallest number of distinct tile types) that uniquely self-assembles the square, answering an open question of Adleman, Cheng, Goel, Huang, Kempe, Moisset de Espanes, and Rothemund ("Combinatorial Optimization Problems in Self-Assembly", STOC 2002). Our investigation leading to this algorithm reveals other positive and negative results about the relationship between the size of a tile system and its "temperature" (the binding strength threshold required for a tile to attach).

==> ptsa.tex <==
\input{main}

==> tam.tex <==
\section{Abstract Tile Assembly Model}
\label{sec-tam-informal}

\newcommand{\fullgridgraph}{G^\mathrm{f}}
\newcommand{\bindinggraph}{G^\mathrm{b}}

This section gives a terse definition of the abstract Tile Assembly Model (aTAM,~\cite{Winf98}). This is not a tutorial; for readers unfamiliar with the aTAM,  \cite{RotWin00} gives an excellent introduction to the model.

Fix an alphabet $\Sigma$. $\Sigma^*$ is the set of finite strings over $\Sigma$.
Given a discrete object $O$, $\langle O \rangle$ denotes a standard encoding of $O$ as an element of $\Sigma^*$.
$\Z$, $\Z^+$, $\N$, $\R^+$ denote the set of integers, positive integers, nonnegative integers, and nonnegative real numbers, respectively.
For all $n \in \N$, $[n]$ denotes the set $\{0, 1, \ldots, n-1\}$.
For a set $A$, $\calP(A)$ denotes the power set of $A$.
Given $A \subseteq \Z^2$, the \emph{full grid graph} of $A$ is the undirected graph $\fullgridgraph_A=(V,E)$, where $V=A$, and for all $u,v\in V$, $\{u,v\} \in E \iff \| u-v\|_2 = 1$; i.e., iff $u$ and $v$ are adjacent on the integer Cartesian plane.
A \emph{shape} is a set $S \subseteq \Z^2$ such that $\fullgridgraph_S$ is connected.
%A shape $S$ is a \emph{tree} if $\fullgridgraph_S$ is acyclic.


A \emph{tile type} is a tuple $t \in (\Sigma^*)^4$; i.e., a unit square with four sides listed in some standardized order, each side having a \emph{glue label} (a.k.a. \emph{glue}) $\ell \in \Sigma^*$.
%consisting of a finite string \emph{label} and nonnegative integer \emph{strength}.
For a set of tile types $T$, let $\Lambda(T)$ denote the set of all glue labels of tile types in $T$.
We assume a finite set $T$ of tile types, but an infinite number of copies of each tile type, each copy referred to as a \emph{tile}. An \emph{assembly}
is a nonempty connected arrangement of tiles on the integer lattice $\Z^2$, i.e., a partial function $\alpha:\Z^2 \dashrightarrow T$ such that $\fullgridgraph_{\dom \alpha}$ is connected and $\dom \alpha \neq \emptyset$. The \emph{shape of $\alpha$} is $\dom \alpha$.
A \emph{strength function} is a function $g:\Lambda(T)\to\N$ indicating, for each glue label $\ell$, the strength $g(\ell)$ with which it binds.
Two adjacent tiles in an assembly \emph{interact} if the glue labels on their abutting sides are equal and have positive strength according to $g$.
Each assembly $\alpha$ induces a \emph{binding graph} $\bindinggraph_\alpha$, a grid graph whose vertices are positions occupied by tiles, with an edge between two vertices if the tiles at those vertices interact.\footnote{For $\fullgridgraph_{\dom \alpha}=(V_{\dom \alpha},E_{\dom \alpha})$ and $\bindinggraph_\alpha=(V_\alpha,E_\alpha)$, $\bindinggraph_\alpha$ is a spanning subgraph of $\fullgridgraph_{\dom \alpha}$: $V_\alpha = V_{\dom \alpha}$ and $E_\alpha \subseteq E_{\dom \alpha}$.}
Given $\tau\in\Z^+$, $\alpha$ is \emph{$\tau$-stable} if every cut of $\bindinggraph_\alpha$ has weight at least $\tau$, where the weight of an edge is the strength of the glue it represents.
That is, $\alpha$ is $\tau$-stable if at least energy $\tau$ is required to separate $\alpha$ into two parts.
When $\tau$ is clear from context, we say $\alpha$ is \emph{stable}.
Given two assemblies $\alpha,\beta:\Z^2 \dashrightarrow T$, we say $\alpha$ is a \emph{subassembly} of $\beta$, and we write $\alpha \sqsubseteq \beta$, if $\dom \alpha \subseteq \dom \beta$ and, for all points $p \in \dom \alpha$, $\alpha(p) = \beta(p)$.





\subsection{Seeded aTAM}
A \emph{seeded tile assembly system} (seeded TAS) is a triple $\calT = (T,\sigma,g,\tau)$, where $T$ is a finite set of tile types, $\sigma:\Z^2 \dashrightarrow T$ is the finite, $\tau$-stable \emph{seed assembly}, $g:\Lambda(T)\to\N$ is the \emph{strength function}, and $\tau\in\Z^+$ is the \emph{temperature}.
Given two $\tau$-stable assemblies $\alpha,\beta:\Z^2 \dashrightarrow T$, we write $\alpha \to_1^{\calT} \beta$ if $\alpha \sqsubseteq \beta$ and $|\dom \beta \setminus \dom \alpha| = 1$. In this case we say $\alpha$ \emph{$\calT$-produces $\beta$ in one step}.\footnote{Intuitively $\alpha \to_1^\calT \beta$ means that $\alpha$ can grow into $\beta$ by the addition of a single tile; the fact that we require both $\alpha$ and $\beta$ to be $\tau$-stable implies in particular that the new tile is able to bind to $\alpha$ with strength at least $\tau$. It is easy to check that had we instead required only $\alpha$ to be $\tau$-stable, and required that the cut of $\beta$ separating $\alpha$ from the new tile has strength at least $\tau$, then this implies that $\beta$ is also $\tau$-stable.}
If $\alpha \to_1^{\calT} \beta$, $ \dom \beta \setminus \dom \alpha=\{p\}$, and $t=\beta(p)$, we write $\beta = \alpha + (p \mapsto t)$.
The \emph{$\calT$-frontier} of $\alpha$ is the set $\partial^\calT \alpha = \bigcup_{\alpha \to_1^\calT \beta} \dom \beta \setminus \dom \alpha$, the set of empty locations at which a tile could stably attach to $\alpha$.
%The \emph{$t$-frontier} $\partial_t \alpha \subseteq \partial \alpha$ of $\alpha$ is the set $\setr{p\in\partial \alpha}{\alpha \to_1^\calT \beta \text{ and } \beta(p)=t}.$

A sequence of $k\in\Z^+ \cup \{\infty\}$ assemblies $\vec{\alpha} = (\alpha_0,\alpha_1,\ldots)$ is a \emph{$\calT$-assembly sequence} if, for all $1 \leq i < k$, $\alpha_{i-1} \to_1^\calT \alpha_{i}$.
We write $\alpha \to^\calT \beta$, and we say $\alpha$ \emph{$\calT$-produces} $\beta$ (in 0 or more steps) if there is a $\calT$-assembly sequence $\vec{\alpha}=(\alpha_0,\alpha_1,\ldots)$ of length $k = |\dom \beta \setminus \dom \alpha| + 1$ such that
1) $\alpha = \alpha_0$,
2) $\dom \beta = \bigcup_{0 \leq i < k} \dom {\alpha_i}$, and
3) for all $0 \leq i < k$, $\alpha_{i} \sqsubseteq \beta$.
In this case, we say that $\beta$ is the \emph{result} of $\vec{\alpha}$, written $\beta=\res{\vec{\alpha}}$.
If $k$ is finite then it is routine to verify that $\res{\vec{\alpha}} = \alpha_{k-1}$.\footnote{If we had defined the relation $\to^\calT$ based on only finite assembly sequences, then $\to^\calT$ would be simply the reflexive, transitive closure $(\to_1^\calT)^*$ of $\to_1^\calT$. But this would mean that no infinite assembly could be produced from a finite assembly, even though there is a well-defined, unique ``limit assembly'' of every infinite assembly sequence.} 
We say $\alpha$ is \emph{$\calT$-producible} if $\sigma \to^\calT \alpha$, and we write $\prodasm{\calT}$ to denote the set of $\calT$-producible assemblies.
The relation $\to^\calT$ is a partial order on $\prodasm{\calT}$ \cite{Roth01,jSSADST}.\footnote{In fact it is a partial order on the set of $\tau$-stable assemblies, including even those that are not $\calT$-producible.}
%Note that all $\calT$-producible assemblies are $\tau$-stable.
A $\calT$-assembly sequence $\alpha_0,\alpha_1,\ldots$ is \emph{fair} if, for all $i$ and all $p\in\partial^\calT\alpha_i$, there exists $j$ such that $\alpha_j(p)$ is defined; i.e., no frontier location is ``starved''.

\newcommand{\w}[1]{\widetilde{#1}}
\newcommand{\wa}{\w{\alpha}}
\newcommand{\wb}{\w{\beta}}
\newcommand{\wg}{\w{\gamma}}

%Given a TAS $\calT=(T,\sigma,\tau)$, an assembly $\alpha$ is \emph{$\calT$-producible}, or \emph{producible} if $\calT$ is clear from context, if either $\alpha = \sigma$, or $\alpha$ results from the $\tau$-stable attachment of a single tile to a producible assembly (``$\tau$-stable attachment'' meaning that the cut separating the tile from the rest of the assembly has strength $\geq \tau$, which implies by induction that $\alpha$ is $\tau$-stable).
An assembly $\alpha$ is \emph{$\calT$-terminal} if $\alpha$ is $\tau$-stable and $\partial^\calT \alpha=\emptyset$.
It is easy to check that an assembly sequence $\vec{\alpha}$ is fair if and only $\res{\vec{\alpha}}$ is terminal.
We write $\termasm{\calT} \subseteq \prodasm{\calT}$ to denote the set of $\calT$-producible, $\calT$-terminal assemblies.
Let $\alpha$ be an assembly, and let $\wa$ denote the set of all assemblies that are equivalent to $\alpha$ up to translation.
We have fixed assemblies at certain positions on $\Z^2$ only for mathematical convenience in some contexts, but of course real assemblies float freely in solution and do not have a fixed position.
For clarity we often abuse notation and take $\alpha$ to be the same object as $\wa$.

A seeded TAS $\calT$ is \emph{directed (a.k.a., deterministic, confluent)} if the poset $(\prodasm{\calT}, \to^\calT)$ is directed; i.e., if for each $\alpha,\beta \in \prodasm{\calT}$, there exists $\gamma\in\prodasm{\calT}$ such that $\alpha \to^\calT \gamma$ and $\beta \to^\calT \gamma$.\footnote{The following two convenient characterizations of ``directed'' are routine to verify.
%It is routine to verify that the following two convenient definitions of ``directed'' are equivalent to the stated definition.
$\calT$ is directed if and only if $|\termasm{\calT}| = 1$ (of course by this we mean that all the terminal assemblies are equivalent up to translation). $\calT$ is \emph{not} directed if and only if there exist $\alpha,\beta\in\prodasm{\calT}$ and $p \in \dom \alpha \cap \dom \beta$ such that $\alpha(p) \neq \beta(p)$.}
We say that a TAS $\calT$ \emph{strictly self-assembles} a shape $S \subseteq \Z^2$ if, for all $\alpha \in \termasm{\calT}$, $\dom \alpha = S$; i.e., if every terminal assembly produced by $\calT$ has shape $S$.
If $\calT$ strictly self-assembles some shape $S$, we say that $\calT$ is \emph{strict}.
Note that the implication ``$\calT$ is directed $\implies$ $\calT$ is strict'' holds, but the converse does not hold.


\subsection{Hierarchical aTAM}
A \emph{hierarchical tile assembly system} (hierarchical TAS) is a triple $\calT = (T,g,\tau)$, where $T$ is a finite set of tile types, $g:\Lambda(T)\to\N$ is the \emph{strength function}, and $\tau\in\Z^+$ is the \emph{temperature}.
Let $\alpha,\beta:\Z^2 \dashrightarrow T$ be two assemblies.
Say that $\alpha$ and $\beta$ are \emph{nonoverlapping} if $\dom\alpha \cap \dom\beta = \emptyset$.
If $\alpha$ and $\beta$ are nonoverlapping assemblies, define $\alpha \cup \beta$ to be the assembly $\gamma$ defined by $\gamma(p) = \alpha(p)$ for all $p\in\dom\alpha$, $\gamma(p) = \beta(p)$ for all $p \in \dom \beta$, and $\gamma(p)$ is undefined for all $p \in \Z^2 \setminus (\dom\alpha \cup \dom\beta)$.
An assembly $\gamma$ is \emph{singular} if $\gamma(p)=t$ for some $p\in\Z^2$ and some $t \in T$ and $\gamma(p')$ is undefined for all $p' \in \Z^2 \setminus \{p\}$.
Given a hierarchical TAS $\calT=(T,g,\tau)$, an assembly $\gamma$ is \emph{$\calT$-producible} if either 1) $\gamma$ is singular, or 2) there exist producible nonoverlapping assemblies $\alpha$ and $\beta$ such that $\gamma = \alpha\cup\beta$ and $\gamma$ is $\tau$-stable.\footnote{Unlike some definitions of the hierarchical aTAM, we have not allowed for translation of $\alpha$ and $\beta$ to determine whether they can stably attach.  This is because every translation of every producible assembly is itself producible.}
In the latter case, write $\alpha + \beta \to \gamma$.
An assembly $\alpha$ is \emph{$\calT$-terminal} if for every producible assembly $\beta$ such that $\alpha$ and $\beta$ are nonoverlapping, $\alpha \cup \beta$ is not $\tau$-stable.\footnote{The restriction on overlap is a model of a chemical phenomenon known as \emph{steric hindrance}~\cite[Section 5.11]{WadeOrganicChemistry91} or, particularly when employed as a design tool for intentional prevention of unwanted binding in synthesized molecules, \emph{steric protection}~\cite{HellerPugh1,HellerPugh2,GotEtAl00}.}
Define $\prodasm{\calT}$ to be the set of all $\calT$-producible assemblies.
Define $\termasm{\calT} \subseteq \prodasm{\calT}$ to be the set of all $\calT$-producible, $\calT$-terminal assemblies.
A hierarchical TAS $\calT$ is \emph{directed (a.k.a., deterministic, confluent)} if $|\termasm{\calT}|=1$.\footnote{Again, technically by this we mean that the quotient set of $\termasm{\calT}$ under the equivalence relation defined by equality under translation is a singleton set.}
We say that a TAS $\calT$ \emph{strictly self-assembles} a shape $S \subseteq \Z^2$ if, for all $\alpha \in \termasm{\calT}$, $\dom \alpha = S$; i.e., if every terminal assembly produced by $\calT$ has shape $S$.

Let $\calT$ be a hierarchical TAS, and let $\alpha \in \prodasm{\calT}$ be a $\calT$-producible assembly.
An \emph{assembly tree} $\Upsilon$ of $\widehat{\alpha}$ is a full binary tree with $|\dom\widehat{\alpha}|$ leaves, whose nodes are labeled by $\calT$-producible assemblies, with $\widehat{\alpha}$ labeling the root, singular assemblies labeling the leaves, and node $u$ labeled with $\gamma$ having children $u_1$ labeled with $\alpha$ and $u_2$ labeled with $\beta$, with the requirement that $\alpha + \beta \to \gamma$.
That is, $\Upsilon$ represents one possible pathway through which $\widehat{\alpha}$ could be produced from individual tile types in $\calT$.
Let $\Upsilon(\calT)$ denote the set of all assembly trees of $\calT$.
Say that an assembly tree is \emph{$\calT$-terminal} if its root is a $\calT$-terminal assembly.
Let $\Upsilon_\Box(\calT)$ denote the set of all $\calT$-terminal assembly trees of $\calT$.
Note that even a directed hierarchical TAS can have multiple terminal assembly trees that all have the same root terminal assembly.




%In this paper we will always use \emph{singly-seeded temperature-2} TAS's, those with $|\dom \sigma|=1$ and $\tau=2$; hence we will use the term \emph{seed tile} for $\sigma$ as well, and for the remainder of this paper we use the term TAS to mean singly-seeded temperature-2 TAS.
When $\calT$ is clear from context, we may omit $\calT$ from the notation above and instead write
$\to_1$,
$\to$,
$\partial \alpha$,
\emph{frontier},
\emph{assembly sequence},
\emph{produces},
\emph{producible}, and
\emph{terminal}.
%Since the behavior of a TAS $\calT=(T,\sigma,2)$ is unchanged if every glue with strength greater than 2 is changed to have strength exactly 2, we assume henceforth that all glue strengths are 0, 1, or 2, and use the terms \emph{null glue}, \emph{single glue}, and \emph{double glue}, respectively, to refer to these three cases.\footnote{We use \emph{null bond}, \emph{single bond}, and \emph{double bond} similarly to refer to the \emph{interaction} of two tiles.}
We also assume without loss of generality that every single glue or double glue occurring in some tile type in some direction also occurs in some tile type in the opposite direction, i.e., there are no ``effectively null'' single or double glues.
%\footnote{Thus the existence of a tile with a double glue facing empty space implies that the empty space is part of the frontier. Many of our arguments use the contrapositive that if a shape $S$ is strictly self-assembled by a tile assembly system and a side of a tile faces a point $p \not\in S$, then the tile cannot have a double glue on that side.}




==> two-handed-assembly-time.tex <==

In this section we define a formal notion of time complexity for hierarchical tile assembly systems, in order to show that the subset of systems known as partial order systems cannot assemble any shape of diameter $N$ in faster than time $\Omega(N)$.
The model we use applies to both the seeded aTAM and the hierarchical aTAM.
For hierarchical systems, our model may not be completely suitable since we make some unrealistic assumptions.\footnote{For example, we ignore diffusion rates of molecules based on size and assume that large assemblies diffuse as fast as individual tiles.
We also assume that the binding energy $\tau$ necessary for a small tile $t$ to attach stably to an assembly $\alpha$ is the same as the binding energy required for a large assembly $\beta$ to attach stably to $\alpha$, even though one would expect such large assemblies to have a higher reverse rate of detachment (slowing the net rate of forward growth) if bound with only strength $\tau$.
}
However, our entire purpose for defining time complexity in the hierarchical aTAM is to show a lower bound, demonstrating that hierarchical partial order systems can proceed no faster than seeded assembly despite the apparent extra parallelism.
Our assumptions will have the effect of making hierarchial self-assembly appear \emph{faster} than if we modeled the underlying chemical kinetics more carefully.
We show that even with these extra assumptions, the time complexity of hierarchical partial order systems is \emph{still} no better than the seeded aTAM.


\opt{submission}{
    \begin{wrapfigure}{r}{2.9in}
    \vspace{-15pt}
      \begin{center}
      \includegraphics[width=2.9in]{figures/two-handed-square-high-level}
      \caption{\label{fig:two-handed-square-high-level} \figuresize
      \FigSquareHighLevelCaption}
      \end{center}
    \vspace{-20pt}
    \end{wrapfigure}
}



\newcommand{\ha}{\widehat{\alpha}}




\subsubsection{Definition of Time Complexity of Directed Seeded Systems}


We now review the definition of time complexity of seeded self-assembly proposed in~\cite{AdChGoHu01}.
A \emph{concentrations function} on a tile set $T$ is a probability measure $C:T \to [0,1]$.
Each tile type $r$ is assumed to be held at a fixed concentration $C(r)$ throughout the process of assembly.\footnote{For singly-seeded tile systems in which the seed tile $s \in T$ appears only once at the origin, this assumption is valid in the limit of low seed concentration $C(s)$ compared to all other concentrations $C(r)$ for $r \in T \setminus \{s\}$.
This is because the number of terminal assemblies (if each is of size at most $K$) will be limited by $C(s)$, implying the percentage change in every other tile type $r$'s concentration is at most $K \cdot C(s) / C(r)$; therefore ``low'' seed concentration means setting $C(s) \ll C(r) / K$ for all $r \in T \setminus\{s\}$.
In fact, to obtain an assembly time asymptotically as fast, one need only ensure that for all $r$, $C(r) \geq 2 \#(r) C(s)$, where $\#(r)$ is the number of times $r$ appears in the terminal assembly $\alpha$.
This guarantees that the concentration of $t$ is always at least half of its start value, which means that the assembly time, each step of which is proportional to the concentration of the tile type attaching at that step, is at most doubled compared to the case when the concentrations are held constant.}
The assembly time for producing a terminal assembly $\ha$ in a seeded TAS $\calT=(T,\sigma,g,\tau)$ is defined by picking a copy of the seed arbitrarily and taking the expected time before the seed grows into $\ha$, conditioned on $\ha$ actually assembling (since there could be other terminal assemblies), when assembly proceeds according to the following stochastic model.
The assembly process is described as a continuous-time Markov process in which each state represents a producible assembly, and the initial state is the seed assembly $\sigma$.
For each pair of producible assemblies $\alpha,\beta$ such that $\alpha \to_1 \beta$ via the addition of tile type $r$, there is a transition in the Markov process from state $\alpha$ to state $\beta$ with transition rate $C(r)$.\footnote{That is, the expected time until the next attachment of a tile to $\alpha$ is an exponential random variable with rate $\sum_{p\in\partial\alpha} C(\ha(p))$, where $\partial\alpha$ is frontier of $\alpha$, the set of empty locations at which a tile could stably attach to $\alpha$.
The probability that a particular $p'\in\partial\alpha$ leading to assembly $\beta$ is the next location of attachment is $C(\ha(p')) / \sum_{p\in\partial\alpha} C(\ha(p))$.}
If $\calT$ is directed, then $\ha$ is the unique sink state of the Markov process.
The time to reach $\ha$ from $\sigma$ is a random variable $\time_{\calT,C}$, and the assembly time complexity of the directed seeded TAS $\calT$ with concentrations $C$ is defined to be $\mathsf{T}(\calT,C) = \exp{\time_{\calT,C}}$.
%Given a finite shape $S\subset \Z^2$, the \emph{(directed) seeded assembly time complexity} of $S$ is $\timeS(S) = \inf_{\calT,C} \mathsf{T}(\calT,C)$, where the infimum is over all directed seeded TAS's $\calT$ that strictly self-assembly $S$ and tile concentration functions $C$ to $\calT$.
%The authors of~\cite{AdChGoHu01} show that $\timeS(S_n) = \Theta(n)$, where $S_n$ is the $n \times n$ square.

The requirement that the tile concentrations function $C$ be a probability measure, rather than an arbitrary measure taking values possibly greater than 1, reflects a physical principle known as the \emph{finite density constraint}, which stipulates that a given unit volume of solution may contain only a bounded number of molecules (if for no other reason than to avoid forming a black hole).
By normalizing so that one ``unit'' of volume is the volume required to fit one tile, we obtain that the total concentration of tiles (concentration defined as  number or mass per unit volume) cannot exceed 1.
By letting their total concentration be exactly 1, we are essentially requiring that the assembly process is carried out in the smallest volume (which leads to the fastest reaction time) required to satisfy the finite density constraint.%, in order to normalize systems for fair comparison.

First, we have the following time complexity lower bound for seeded systems, which strengthens and implies Lemma 4.6 of the full version of~\cite{AdChGoHu01}, which applies only to directed systems.
\opt{submission}{A proof of Theorem~\ref{thm-seeded-time-lower-bound} is contained in Section~\ref{sec-app-hier-partial-order-slow}.}
This theorem says that even for non-directed systems, a seeded TAS can still grow its diameter only linearly with time.
Let $d \in \Z^+$.
Let $\calT=(T,\sigma,g,\tau)$ be a singly-seeded TAS (meaning $|\dom\sigma|=1$), and let $C:T\to[0,1]$ be a concentrations function.
Since it takes only constant time for the assembly to grow to any constant radius, restricting attention to singly-seeded systems does not asymptotically affect the result for tile systems with a finite seed assembly of size larger than 1.
%We say that $\calT$ is \emph{$d$-wide} if, for all $\ha \in \termasm{\calT}$, some point in $\dom \ha$ is at least distance $d$ (in the $L_1$ norm) from the seed.
%In other words, we require that $\calT$ is guaranteed to grow to at least distance $d$ from the seed.\footnote{Otherwise it does not make sense to ask how long it takes to grow to distance $d$.  Alternately, we could have formulated the statement as the expected time to grow to distance $d$, conditioned on the event that growth ever reaches distance $d$, but }
Let $\mathbf{D}(\calT,C,d)$ be the random variable representing the time that any tile is first placed at distance $d$ from the seed, conditioned on the event that a tile is eventually placed at least distance $d$ (in the $L_1$ norm) from the seed, with $\mathbf{D}(\calT,C,d)=\infty$ if all producible, terminal assemblies of $\calT$ are completely contained in radius $d-1$ around the seed.

\begin{theorem}\label{thm-seeded-time-lower-bound}
For each $d \in \Z^+$, each singly-seeded TAS $\calT$, and each concentrations function $C:T\to[0,1]$, $\exp{\mathbf{D}(\calT,C,d)} \geq \Omega(d)$.
\end{theorem}

\newcommand{\ProofSeededTimeLowerBound}{
    Since we care only about the first time at which a tile is attached at distance $d$ (before which there are no tiles at distance $d'$ for any $d' \geq d$), we can restrict the assembly process to the region of radius $d$ around the seed.
    Therefore we model the assembly process as if it proceeds normally until the first tile attaches at distance $d$ from the seed, at which point all growth immediately halts.
    %We state the proof only for \emph{singly-seeded} tile systems, meaning those with a single seed tile.

    Define $\R^+ = [0,\infty)$.
    Given $i \in \{0,\ldots,d\}$ and $t \in \R^+$, let $\mathbf{X}_i(t)$ be a random variable denoting the number of tiles attached at locations with distance exactly $i$ from the seed at time $t$, under the restriction stated above that all assembly halts the moment that a tile is placed at distance $d$.
    Then for all $t\in\R^+$, the event $\mathbf{X}_d(t) = 0$ (no tile is at distance $d$ by the time $t$) is equivalent to the event $\mathbf{D}(\calT,C,d) > t$ (the time of the first attachment at distance $d$ strictly exceeds $t$).
    %Once this time has passed, the variables $X_i(t)$ no longer model the assembly process accurately, but since we

    %Note that if $\calT$ cannot grow to distance $i > d$, then $\mathbf{X}_i(t) = 0$ for all $t\in\R^+$.
    In a seeded TAS, tiles can attach at a location only when there is another tile adjacent to the location.
    Locations at $L_1$-distance $i$ to the seed are only adjacent to locations at distance either $i+1$ or $i-1$ to the seed.
    Off the $x$- and $y$-axes, each location at distance $i$ has two neighbors at distance $i-1$ and two neighbors at distance $i+1$, and for the 4 locations at distance $i$ on either axis, every location has one neighbor at distance $i-1$ and three neighbors at distance $i+1$.
    Therefore, at time $t$, tiles are attachable to at most $3 \mathbf{X}_{i-1}(t) + 2 \mathbf{X}_{i+1}(t)$ different locations with distance $i$ to the seed.
    %Let $\alpha$ be an assembly, let $p \in \partial \alpha$, and let $\{\beta_1,\ldots,\beta_k\}$ denote the set of assemblies such that $\alpha \to_1 \beta_i$ via attachment at location $p$.
    %Since $\sum_{r \in T} C(r) = 1$, this implies that the rate of attachment to $\alpha$ at location $p$ is $\sum_{}$.
    Since the total concentration of single tiles is $1$, the rate at which tiles attach at any given location is at most $1$.
    For all $i\in\{0,\ldots,d\}$, define the function $f_i:\R^+ \to \R^+$ for all $t\in\R^+$ by $f_i(t) = \exp{\mathbf{X}_i(t)}$.
    Then for $i\in\{1,\ldots,d-1\}$,
    \[
    \frac{df_i(t)}{dt}\ \leq\ 3f_{i-1}(t)\ +\ 2f_{i+1}(t),
    %\]
    \text{ and }
    %\[
    \frac{df_d(t)}{dt}\ \leq\ 3f_{d-1}(t).
    \]
    The lack of a $2f_{d+1}(t)$ term in the latter inequality is due to our modification of the assembly process to immediately halt once the first tile attaches at distance $d$.
    Since the assembly process always starts with a single seed tile, $f_0(t)=1$ for all $t\in\R^+$, and $f_i(0) = 0$ for all $i \in \{0,\ldots,d\}$.
    For all $t\in\R^+$ and all $i\in\{1,\ldots,d\}$, $f_i(t) \leq 4i$ since there are exactly $4i$ locations at distance exactly $i$ to the seed.
    %To prove the theorem, we only need to focus on when the first tile attaches at distance $d$. Until that time, no tile will be able to attach at distance larger than $d$.

    Let $t_0 \in \R^+$ be the unique time at which $f_d(t_0) = \frac{1}{2}.$
    This time is unique since $f_d$ is monotonically increasing.
    Since $f_d(t_0) = \exp{\mathbf{X}_d(t_0)}$, by Markov's inequality, $\prob[\mathbf{X}_d(t_0) \geq 1] \leq \frac{1}{2}$, implying that $\prob[\mathbf{X}_d(t_0) < 1] > \frac{1}{2}$.
    Since $\mathbf{X}_d$ is integer-valued and nonnegative, this is equivalent to stating that $\prob[\mathbf{X}_d(t_0) = 0] > \frac{1}{2}$.
    Recall that $\mathbf{X}_d(t_0) = 0 \iff \mathbf{D}(\calT,C,d) > t_0$,  whence $\prob[\mathbf{D}(\calT,C,d) > t_0] > \frac{1}{2}$.
    By Markov's inequality, $\exp{\mathbf{D}(\calT,C,d)} > \frac{t_0}{2}$.
    Thus it suffices to prove that $t_0 \geq \Omega(d)$.
    To do this, we define a simpler function that is an upper bound for $f_d$ and solve its differential equations.

    %Since this means that if we do not allow tiles to attach at distance $d+1$ or more, then at least half of the instances, no tiles attach at distance $d$ within time $\frac{d}{c}$ and thus the average time for any tile to attach at distance $d$ to the seed is at least $\frac{d}{2c}$. In the rest of the proof, we focus on giving an upper bound on $f_d(t)$ subject to $f_{i}(t) = 0$ for all $t$ and all $i >d$.

    For all $i\in\{0,\ldots,d\}$, define the function $g_i:\R^+ \to \R^+$ (which will serve as an upper bound for $f_i$) as follows.
    For all $1\in\{1,\ldots,d-1\}$,
    \[
    \frac{dg_i(t)}{dt}\ =\ 3g_{i-1}(t)\ +\ 2g_{i+1}(t),\ \mbox{when $g_i(t) < 4d$},
    \]
    \[
    \frac{dg_d(t)}{dt}\ =\ 3g_{d-1}(t),\ \mbox{when $g_d(t) < 4d$},
    \]
    and for all $i\in\{0,\ldots,d\}$,
    \[
    \frac{dg_i(t)}{dt}\ =\ 0,\ \mbox{when $g_i(t) = 4d$},
    \]
    with the boundary conditions $g_0(t)=4d$ for all $t \in \R^+$, $g_i(0) = 0$ for all $i \in \{1,\ldots,d\}$.
    It is routine to check that $g_i(t) \geq f_i(t)$ for all $i\in\{0,\ldots,d\}$ and $t\in\R^+$. Furthermore, if $g_i(t_0) > g_{i+1}(t_0)$ for all $i\in\{0,\ldots,d\}$ and a specific time point $t_0 \in \R^+$, then
    \[
    \frac{dg_i(t)}{dt}\ \geq\ \frac{dg_{i+1}(t)}{dt}\ \mbox{at time $t_0$},
    \]
    Since $g_i(0) \geq g_{i+1}(0)$ for all $i\in\{0,\ldots,d\}$ by definition, we know that $g_i(t) \geq g_{i+1}(t)$ for all $i\in\{0,\ldots,d\}$ and all $t\in\R^+$.
    Using this monotonicity, we can define a set of functions $h_i(t)$ that are upper bounds for $g_i(t)$ by the following.
    \[
    \frac{dh_i(t)}{dt}\ =\ 5h_{i-1}(t) \mbox{, for all $i\in\{1,\ldots,d\}$}, \text{ and } \frac{dh_0(t)}{dt} = 0,
    \]
    with boundary conditions $h_0(t)=4d$ for all $t\in\R^+$, $h_i(0) = 0$ for all $i\in\{0,\ldots,d\}$. Solving these differential equations, we obtain $h_d(t)=\frac{4d}{d!}(5t)^d$.  Letting $t'=\frac{d}{10e}$, by Stirling's inequality $d! > \sqrt{2 \pi d} \left( \frac{d}{e} \right)^d e^{1 / (12 d + 1)} > \left( \frac{d}{e} \right)^d$, we have
    \[
    f_d\left(t'\right)
    \leq
    g_d\left(t'\right)
    \leq
    h_d\left(t'\right)
    =
    \frac{4d}{d!} \cdot \left(5t'\right)^d
    =
    \frac{4d}{d!} \cdot \left( \frac{d}{2 e} \right)^d
    <
    \frac{4d}{\left( \frac{d}{e} \right)^d} \cdot \left( \frac{d}{2 e} \right)^d
    =
    \frac{4d}{2^d}.
    \]
    %The last inequality follows from Stirling's inequality $d! > \sqrt{2 \pi d} \left( \frac{d}{e} \right)^d e^{1 / (12 d + 1)}$.
    Since $f_d$ is monotonically increasing, $f_d(t_0) = \frac{1}{2}$ by definition, and $\frac{4d}{2^d} < \frac{1}{2}$ for sufficiently large $d$, this implies that $t_0 > t' = \frac{d}{10e}$.
}

\opt{normal}{
    \begin{proof}
      \ProofSeededTimeLowerBound
    \end{proof}
}



\subsubsection{Definition of Time Complexity of Directed Hierarchical Systems}


To define time complexity for hierarchical systems, we employ more explicitly the chemical kinetics implicitly underlying the above time complexity model for seeded systems.
We treat each assembly as a single molecule. If two assemblies $\ta$ and $\tb$ can attach to create a assembly $\tg$, then we model this as a chemical reaction $\ta + \tb \to \tg$, in which the rate constant is assumed to be equal for all reactions (and normalized to 1).
Note in particular that if $\ta$ and $\tb$ can be attached in two different ways, this is modeled as two different reactions, even if both result in the same assembly.\footnote{The fact that some directed systems may not require at least one of these attachments to happen in every terminal assembly tree is the reason we impose the partial order requirement when proving our time complexity lower bound.}

We would like to analyze the assembly time in such as way as to facilitate direct comparison with the results of~\cite{AdChGoHu01}.
With a stochastic model such as Gillespie's algorithm~\cite{Gillespie77,GibsonBruck00,Gillespie07} using finite tile counts, it is possible that no copy of the terminal assembly forms, so it is not clear how to sensibly ask how long it takes to form.\footnote{This problem is easily averted in a seeded system by setting the seed concentration sufficiently low (but still $\Omega(|T|)$).  In a hierarchical system it is not clear how to avoid this problem.}
The mass-action model of kinetics~\cite{epstein1998introduction} describes concentrations as a dynamical system that evolves continuously over time according to ordinary differential equations derived from reaction rates.
In the mass-action model, the terminal assembly is guaranteed to form, which resolves one issue with the purely stochastic model; however, some (low) concentration of the terminal assembly forms in the first infinitesimal amount of time.
It is not clear how to define the time to assemble the terminal assembly $\ha$.
Some choices such as measuring the time to half-completion (time required for the concentration of $\ha$ to exceed half of its steady-state concentration) are potentially subject to ``cheats'' such as systems that ``kill'' all but the fastest growing assemblies so as to artificially inflate the average time to completion of those that successfully assemble into the terminal assembly.

The model of assembly time that we define is a continuous-time stochastic model similar to that of~\cite{AdChGoHu01}.
However, rather than fixing transition rates at each time $t\in\R^+$ as constant, we use mass-action kinetics to describe the evolution over time of the concentration of producible assemblies, including individual tile types, which in turn determine transition rates.
To measure the time to complete a terminal assembly, we use the same stochastic model as~\cite{AdChGoHu01}, which fixes attention on one particular tile and asks what is the expected time for it to grow into the terminal assembly, where the rate of attachment events that grow it are time-dependent, governed by the continuous mass-action evolution of concentration of assemblies that could attach to it.
Note in particular that unlike the seeded model, we allow the tile concentrations to deplete, since it is no longer realistic (or desirable for nontrivial hierarchical constructions) to assume that individual tiles do not react until they encounter the single assembly containing the seed.
Like the model of~\cite{AdChGoHu01}, we define assembly time only for directed systems, in order to meaningfully ask the question ``How long until terminal assembly $\ha$ forms?'' without having to deal with the possibility that $\ha$ does not form.





Let $\calT=(T,g,\tau)$ be a (possibly non-directed) hierarchical TAS, and let $C:T\to[0,1]$ be a concentrations function.
Let $\R^+ = [0,\infty)$, and let $t\in\R^+.$
Let $[\alpha](t)$ denote the concentration of $\alpha$ at time $t$, defined as follows.\footnote{More precisely, $[\alpha](t)$ denotes the concentration of the equivalence class of assemblies that are equivalent to $\alpha$ up to translation.  We have defined assemblies to have a fixed position only for mathematical convenience in some contexts, but for defining concentration, it makes no sense to allow the concentration of an assembly to be different from one of its translations.}
If $\alpha$ is consumed in reactions $\alpha + \beta_1 \to \gamma_1, \ldots, \alpha + \beta_n \to \gamma_n$ and produced in reactions $\beta'_1 + \gamma'_1 \to \alpha, \ldots, \beta'_m + \gamma'_m \to \alpha$, then the concentration $[\alpha](t)$ of $\alpha$ at time $t$ is described by the differential equation
\begin{equation}\label{eq-conc-diff}
    \frac{d [\alpha](t)}{d t} = \sum_{i=1}^m [\beta'_i](t) [\gamma'_i](t) - \sum_{i=1}^n [\alpha](t) [\beta_i](t),
\end{equation}
and similarly for all other producible assemblies, with $[\alpha](0) = C(r)$ if $\alpha$ is an assembly consisting of a single tile $r$, and $[\alpha](0) = 0$ otherwise.
This completes the definition of the dynamics of concentrations of producible assemblies; it remains to define the time complexity of assembling the terminal assembly of directed systems.

Suppose $\calT$ is directed.
Then let $\ha\in\termasm{\calT}$ be its unique producible, terminal assembly.
Although we have distinguished between seeded and hierarchical systems, for the purpose of defining a model of time complexity in hierarchical systems and comparing them to the seeded system time complexity model of~\cite{AdChGoHu01}, it is convenient to introduce a ``seed'' tile into the hierarchical system, in order to stochastically analyze the growth of this tile when it reacts in a solution that is itself evolving according to the continuous model described above.
The seed does not have the purpose of nucleating growth, but is introduced merely to focus attention on a single molecule that has not yet assembled anything, in order to ask how long it will take to assemble into the final terminal assembly.\footnote{For our lower bound result, it will not matter which location is selected as the timekeeper, except in the following sense.  We define partial order systems, the class of hierarchical TAS's to which the bound applies, also with respect to a particular ``seed'' location $p$.  A TAS may be a partial order system with respect to one location but not another, but for all locations $p$ for which the TAS is a partial order system, the time lower bound applies when $p$ is selected as the timekeeper.}
Let $\ha$ be the unique terminal assembly of the hierarchical TAS.
We choose a copy of a tile type $s$ at position $p\in\dom\ha$ to designate as a ``timekeeper seed''.
The assembly of $s$ into $\ha$ is described as a time-dependent continuous-time Markov process in which each state represents a producible assembly defined at $p$, and the initial state is the assembly with only $s$ at position $p$.
For each state $\alpha$ representing a producible assembly with $s$ at the origin, and for each pair of producible assemblies $\beta,\gamma$ such that $\alpha + \beta \to \gamma$ (with the translation assumed to happen only to $\beta$ so that $\alpha$ stays ``fixed'' in position), there is a transition in the Markov process from state $\alpha$ to state $\gamma$ with transition rate $[\beta](t)$.\footnote{That is, for the purpose of determining the continuous dynamic evolution of the concentration of assemblies, including $\alpha$,  in solution at time $t$, the rate of the reaction $\alpha + \beta \to \gamma$ at time $t$ is assumed to be proportional to $[\alpha](t)[\beta](t)$.
However, for the purpose of determining the stochastic dynamic evolution of one particular copy of $s$, the rate of this reaction at time $t$ is assumed to be proportional only to $[\beta](t)$.
This is because we want to describe the rate at which \emph{this particular copy} of $\alpha$, the one containing the copy of $s$ at position $p$ that we fixed at time 0, encounters assemblies of type $\beta$.
This instantaneous rate is independent of the number of other copies of $\alpha$ at time $t$ (although after $\epsilon$ seconds the rate will change to $[\beta](t+\epsilon)$, which of course \emph{will} depend on $[\alpha]$ over that time interval).}
Note that unlike the seeded model, the transition rates vary over time since the assemblies (including assemblies that are individual tiles) with which $s$ could interact are themselves being produced and consumed.
In particular, tile concentrations are not assumed to be held constant, since we can no longer assume that tiles have no interaction except with the single assembly containing the seed.


We define $\time_{\calT,C,p}$ to be the random variable representing the time taken for the copy of $s$ at position $p$ to assemble into $\ha$ via some sequence of reactions as defined above.
Note in particular that unlike the seeded model, there are other reactions occurring outside the sequence, between two assemblies $\alpha$ and $\beta$ that do not contain the timekeeper tile.
However, these (continuously modeled) reactions will determine the concentration of tiles and assemblies that in turn determine the propensities of (stochastically modeled) reactions that \emph{do} involve the timekeeper.
We define the time complexity of a directed hierarchical TAS $\calT$ with concentrations $C$ and timekeeper location $p$ to be $\mathsf{T}(\calT,C,p) = \exp{\time_{\calT,C,p}}$.
%Given a finite shape $S\subset \Z^2$, the \emph{(directed) hierarchical assembly time complexity} of $S$ is $\timeH(S) = \inf_{\calT,C} \max_{p\in\dom\ha(\calT)} \mathsf{T}(\calT,C,p)$, where the infimum is over all directed hierarchical TAS's $\calT$ that strictly self-assembly $S$, tile concentration functions $C$ to $\calT$, and $\ha(\calT)$ is defined to be the unique terminal assembly of $\calT$.


We note in particular that our construction of Theorem~\ref{thm-hierarchical-square} is composed of $(\frac{n}{\log n})^2$ different types of $O(\log n) \times O(\log n)$ ``blocks'' that can each grow via only one reaction.
At least one of these blocks $\beta$ must obey $[\beta](t) \leq \frac{\log^2 n}{n^2}$ for all $t\in\R^+$.
This implies that the rate of the slowest such reaction is at most $\frac{\log^2 n}{n^2}.$
Thus our square construction assembles in at least $\Omega(\frac{n^2}{\log^2 n})$ time, slower than the optimal seeded time of $O(n)$ \cite{AdChGoHu01}.


\subsubsection{Definition of Hierarchical Partial Order Systems}

We will show a lower bound on time complexity for a special class of hierarchical directed TAS's known as \emph{partial order systems}.
Seeded partial order systems were first defined by Adleman, Cheng, Goel, and Huang~\cite{AdChGoHu01} for the purpose of analyzing the running time of their optimal square construction.
Intuitively, a seeded directed TAS with unique terminal assembly $\ha$ is a partial order system if every pair of adjacent positions $p_1$ and $p_2$ in $\ha$ that interact with positive strength have the property that either $p_1$ always receives a tile before $p_2$, or vice versa.
We extend the definition of partial order systems to hierarchical systems in the following way.

Let $\calT=(T,g,\tau)$ be a hierarchical directed TAS with unique terminal assembly $\ha\in\termasm{\calT}$.
%A \emph{terminal assembly tree} of $\ha$ is a full binary tree with $|\dom\ha|$ leaves, in which each leaf is labeled with an assembly consisting of a single tile, the root is labeled with $\ha$, and each internal node is labeled with an assembly producible in one step from the $\tau$-stable attachment of its two child assemblies.
%Note that even a directed hierarchical TAS may have more than one assembly tree of the terminal assembly $\ha$.
Let $\Upsilon$ be any terminal assembly tree of $\calT$.
Let $p\in\dom\ha$ and let $s=\ha(p)$.
The \emph{assembly sequence with respect to $\Upsilon$ starting at $p$} is the sequence of assemblies $\vec{\alpha}_{p,\Upsilon} = (\alpha_1,\ldots,\alpha_k)$ that represent the path from the leaf corresponding to $p$ to the root of $\Upsilon$, so that $\alpha_1$ is the single tile $s$ at position $p$, and $\alpha_k = \ha$.\footnote{That is, $\vec{\alpha}$ is like a seeded assembly sequence in that each $\alpha_i$ is a \emph{subassembly} of $\alpha_{i+1}$ (written $\alpha_i \sqsubseteq \alpha_{i+1}$, meaning $\dom\alpha_i \subseteq \dom\alpha_{i+1}$ and $\alpha_{i}(p) = \alpha_{i+1}(p)$ for all $p \in \dom\alpha_{i}$).
The difference is that $\alpha_i$ and $\alpha_{i+1}$ may differ in size by more than one tile, since $\dom \alpha_{i+1} \setminus \dom\alpha_i$ will consist of all points in the domain of $\alpha_i$'s sibling in $\Upsilon$.}
An \emph{assembly sequence starting at $p$} is an assembly sequence with respect to $\Upsilon$ starting at $p$, for some valid assembly tree $\Upsilon$.

An \emph{attachment preorder} with respect to $p\in\dom\ha$ is a preorder $\preceq$ on $\dom \ha$ such that the following holds:
\begin{enumerate}

  \item For every $p_1,p_2\in\dom\ha$, if and only if $p_1 \preceq p_2$, then for every assembly sequence $\vec{\alpha}=(\alpha_1,\ldots,\alpha_k)$ starting at $p$, for all $1 \leq i \leq k$, ($\alpha_i(p_2)$ is defined $\implies$ $\alpha_i(p_1)$ is defined).
      In other words, $p_1$ must always have a tile by the time $p_2$ has a tile. (Perhaps they always arrive at the same time in every assembly sequence starting at $p$.)

  \item For every pair of adjacent positions $p_1,p_2 \in \dom\ha$, if the tiles at positions $p_1$ and $p_2$ interact with positive strength in $\ha$, then $p_1 \preceq p_2$ or $p_2 \preceq p_1$ (or both).
\end{enumerate}

%TODO: add figures showing intuition of partial order systems


We say that a directed hierarchical TAS $\calT$ with unique terminal assembly $\ha$ is a \emph{hierarchical partial order system with respect to $p$} if it has an attachment preorder with respect to $p$. % for some $p \in \dom\ha$.
%Say that $\calT$ is a partial order system starting at $p$.
If two tiles always arrive at the same time to the assembly containing $p$, then they will be in the same equivalence class induced by $\preceq$.
Given an attachment preorder $\preceq$, we define the \emph{attachment (strict) partial order $\prec$ induced by $\preceq$} to be the partial order on the quotient set of equivalence classes induced by $\preceq$.
In other words, if some subassembly $\alpha \sqsubseteq \ha$ always attaches to the assembly containing $p$ all at once, then all positions $p' \in \dom\alpha$ will be equivalent under $\preceq$.\footnote{More generally, if there is a subset $X\subset \dom\ha$ such that all assemblies $\alpha$ attaching to the assembly containing $p$ have the property that $\dom\alpha \cap X \implies X \subseteq \dom\alpha$.}
It is these equivalence classes of positions that are related under $\prec$.
%Since there is a unique terminal assembly determining which tile types are placed at each position in $\dom\ha$, we may equivalently view these equivalence classes of positions as assemblies

Each attachment partial order $\prec$ induces a directed acyclic graph $G=(V,E)$, where $V = \{\alpha_1,\ldots,\alpha_k\}$, where each $\alpha_i$ represents the subassembly corresponding to some set of positions in $\dom\alpha$ that are equivalent under $\preceq$, and $(\alpha_i,\alpha_j) \in E$ if $\dom\alpha_i \prec \dom\alpha_j$.
In the case of seeded assembly, in which each attachment is of a ``subassembly'' containing a single tile to a subassembly containing the seed, this definition of partial order system is equivalent to the definition of partial order system given in~\cite{AdChGoHu01}.
It is routine to check that the TAS described in Section~\ref{sec-hierarchical-square} is a partial order system, using one of the orange tiles in the upper-left of Figure~\ref{fig:two-handed-square-block} as a ``seed.''



\subsubsection{Time Complexity Lower Bound for Hierarchical Partial Order Systems}

Theorem~\ref{thm-hier-partial-order-slow} establishes that hierarchical partial order systems, like their seeded counterparts, cannot assemble a shape of diameter $N$ in less than $\Omega(N)$ time.
Intuitively, this is proven by using the fact that an attaching assembly of size $K$, which is able to increase the size of the growing assembly by $K$ tiles in a single step, can have concentration at most $\frac{1}{K}$ by conservation of mass, slowing down its rate of attachment (compared to the rate of a single tile) by factor at least $K$, precisely enough to cancel out the potential speedup over a single tile due to its size.
This simplistic argument is not quite accurate and must be amortized over all assemblies that could extend the growing assembly since the growing assembly may be extended at a single attachment site by more than one assembly, but the more assemblies that could extend it, the less the total concentration of the assemblies that could attach to create the extension.
Intuitively, the property of having a partial order on binding subassemblies ensures that the assembly of each path in the partial order graph proceeds by a series of rate-limiting steps, which allows to us prove the theorem by proving upper bounds on each of these rates using this concentration argument.\footnote{The same assembly $\alpha$ could attach to many locations $p_1,\ldots,p_n$.
In a TAS that is not a partial order system, it could be the case that there is not a fixed attachment location that is necessarily required to complete the assembly.
In this case complete assembly might be possible even if only one of $p_1,\ldots,p_n$ receives the attachment of $\alpha$.
Since the minimum of $n$ exponential random variables with rate $1/K$ is itself exponential with rate $n/K$, the very first attachment of $\alpha$ to any of $p_1,\ldots,p_n$ happens in expected time $K/n$, as opposed to expected time $K$ for $\alpha$ to attach to a \emph{particular} $p_i$.
This prevents our technique from applying to such systems.
It is open whether TAS's that are not partial order systems are subject to the same time complexity lower bound.}

\opt{submission}{
    A proof of Theorem~\ref{thm-hier-partial-order-slow} is given in Section~\ref{sec-app-hier-partial-order-slow}.
}

\newcommand{\LemmaConserveMass}{

The following is a ``mass conservation lemma'' that will be helpful in the proof of Theorem~\ref{thm-hier-partial-order-slow}.
Note that it applies to any hierarchical system.
%Define $\R^+ = [0,\infty)$.

\begin{lemma}\label{lem-constant-sum-conc}
  Let $\calT=(T,g,\tau)$ be a hierarchial TAS and let $C:T\to[0,1]$ be a concentrations function. Then for all $t \in \R^+$,
  \[
  \sum_{\alpha \in \prodasm{\calT}} [\alpha](t) \cdot |\alpha| = 1.
  \]
  %where $[\alpha](t)$ is the concentration of assembly $\alpha$ at time $t$.
\end{lemma}

\begin{proof}
  For all $t\in\R^+$, define $f(t) = \sum_{\alpha \in \prodasm{\calT}} [\alpha](t) \cdot |\alpha|.$
  According to our model, $[\alpha](0) = C(r)$ if $\alpha$ consists of a single tile type $r$ and $[\alpha](0)=0$ otherwise, so $f(0) = \sum_{r \in T} C(r) = 1$.
  Therefore it is sufficient (and necessary) to show that $\frac{df}{dt} = 0$.
  For all $\alpha \in \prodasm{\calT}$ and $t\in\R^+$, define $f_\alpha(t) = [\alpha](t) \cdot |\alpha|$.
  Then by \eqref{eq-conc-diff}, and recalling the definitions of $m$, $n$, $\beta'_i$, $\gamma'_i$, and $\beta_i$, annotated as $m(\alpha), n(\alpha)$, etc. to show their dependence on $\alpha$, we have
  \[
    \frac{d f_\alpha}{dt} = |\alpha| \cdot \left( \sum_{i=1}^{m(\alpha)} [\beta'_i(\alpha)](t) \cdot [\gamma'_i(\alpha)](t) - \sum_{i=1}^{n(\alpha)} [\alpha](t) \cdot [\beta_i(\alpha)](t) \right).
  \]
  Then
  \begin{eqnarray*}
    \frac{df}{dt}
    &=&
    \frac{d}{dt} \sum_{\alpha \in \prodasm{\calT}} f_\alpha(t)
    %\\&=&
    =
    \sum_{\alpha \in \prodasm{\calT}} \frac{d f_\alpha}{dt}
    \\&=&
    %=
    \sum_{\alpha \in \prodasm{\calT}} \left( \sum_{i=1}^{m(\alpha)} |\alpha| \cdot [\beta'_i(\alpha)](t) \cdot [\gamma'_i(\alpha)](t) - \sum_{i=1}^{n(\alpha)} |\alpha| \cdot [\alpha](t) \cdot [\beta_i(\alpha)](t) \right).
  \end{eqnarray*}
  Let $\mathcal{R}$ denote the set of all attachment reactions of $\calT$, writing $R(\alpha,\beta,\gamma)$ to denote the reaction $\alpha + \beta \to \gamma$.
  Note that for each such reaction, $|\alpha| + |\beta| = |\gamma|$.
  Note also that each such reaction contributes precisely three unique terms in the last expression above, two negative (of the form $- |\alpha| [\alpha](t) [\beta](t)$ and $-|\beta| [\alpha](t) [\beta](t)$) and one positive (of the form $|\gamma| [\alpha](t) [\beta](t)$).

  Then
  \begin{align*}
    \frac{df}{dt}
    &=
    \sum_{R(\alpha,\beta,\gamma) \in \mathcal{R}} \left(|\gamma| \cdot [\alpha](t) \cdot [\beta](t) - |\alpha| \cdot [\alpha](t) \cdot [\beta](t) - |\beta| \cdot [\alpha](t) \cdot [\beta](t) \right)
    \\&=
    \sum_{R(\alpha,\beta,\gamma) \in \mathcal{R}} (|\gamma| - |\alpha| - |\beta|) \cdot [\alpha](t) \cdot [\beta](t)
    =
    \sum_{R(\alpha,\beta,\gamma) \in \mathcal{R}} 0 \cdot [\alpha](t) \cdot [\beta](t)
    =
    0. \qedhere
  \end{align*}
  %Each reaction of the form $\alpha+\beta\to\gamma$ consumes an assembly with $|\alpha|$ tiles and another assembly with $|\beta|$ tiles, and produces an assembly with $|\gamma| = |\alpha| + |\beta|$ tiles.
%  Therefore, the quantity
%  $
%    |\alpha| \cdot [\alpha] + |\beta| \cdot [\beta] + |\gamma| \cdot [\gamma]
%  $
%  is preserved by this reaction.
%  This implies that the sum of all such terms for all producible assemblies is constant over time, and equal to the initial quantity
%  \[
%    \sum_{\alpha \in \prodasm{\calT}} [\alpha](0) \cdot |\alpha|
%    =
%    \sum_{r \in T} C(r) = 1. \qedhere
%  \]
\end{proof}
}

\opt{normal}{\LemmaConserveMass}

\begin{theorem} \label{thm-hier-partial-order-slow}
  Let $\calT=(T,g,\tau)$ be a hierarchial partial order system starting at $p\in\Z^2$, with
  unique
  terminal assembly of diameter $N$.
  Then for all concentration functions $C:T\to[0,1]$, $\mathsf{T}(\calT,C,p) \geq \Omega(N)$.
\end{theorem}

\newcommand{\ProofHierPartialOrderSlow}{
  Let $\ha\in\termasm{\calT}$ be the unique terminal assembly of $\calT$.
  Let $\preceq$ be the attachment preorder testifying to the fact that $\calT$ is a partial order system.
  Let $\prec$ be the strict partial order induced by $\preceq$.
  Let $G=(V,E)$ be the directed acyclic graph induced by $\prec$, with $V = \{\alpha_1,\ldots,\alpha_k\}$.
  Assign weights to the edges of $E$ by $w(\alpha_i,\alpha_j) = |\dom\alpha_j|$.
  If $P$ is a longest weighted path in $G$, it must be the case that $w(P) \geq N/2$.


  Let $P = (\alpha'_1,\ldots,\alpha'_l)$ be any path in $G$, with weight $w(P) = \sum_{i=2}^l |\alpha'_i|$, with $\alpha'_1$ being the single tile at position $p$.
  Because of the precedence relationship described by $\prec$, no portion of the path $P$ can form until its immediate predecessor on $P$ is present.
  It suffices to show that $w(P) \leq O(\exp{\time_{\calT,C,p}})$.
  Let $\mathbf{T}_P$ be the random variable representing the time taken for the complete path $P$ to form.
  It is clear that $\mathbf{T}_P \leq \time_{\calT,C,p}$.
  We will show that $\exp{\mathbf{T}_P} \geq \Omega(w(P))$.


  To show that $\exp{\mathbf{T}_P} \geq \Omega(w(P))$, we will show that for all $t\in\R^+$, $\exp{\mathbf{L}(t)} \leq t$.
  This will suffice because of the following argument.
  After some amount of time, some prefix $P'$ of the path $P$ has assembled (possibly with some other portions of $\ha$ not on the path $P$).
  Given $t\in\R^+$, let $\mathbf{L}(t)$ be the random variable indicating the weighted length of this prefix after $t$ seconds.
  By Markov's inequality, $\prob[\mathbf{L}(t) \geq 2t] \leq \frac{1}{2}$.
  Letting $t=w(P)/2$, the event $\mathbf{L}(w(P)/2) \geq w(P)$ is equivalent to the event $\mathbf{T}_{P} \leq w(P)/2.$
  Thus $\prob[\mathbf{T}_{P} \leq w(P)/2] \leq \frac{1}{2}.$
  By Markov's inequality, $\exp{\mathbf{T}_{P}} \geq w(P) / 4 = \Omega(w(P)),$ which establishes the theorem.

  It remains to show that for all $t\in\R^+$, $\exp{\mathbf{L}(t)} \leq t$.
  Define the function $f:\R^+ \to \R^+$ for all $t\in\R^+$ by $f(t) = \exp{\mathbf{L}(t)}$, noting that $f(0)=0$.
  Let $f' = \frac{d f}{d t}$.
  It suffices to show that for all $t\in\R^+$, $f'(t) \leq 1$.

  Let $P' = (\alpha'_1, \ldots, \alpha'_{m'})$ be the prefix of $P$ formed after $t$ seconds.  Let $\beta_1, \beta_2, \ldots, \beta_{m}$, with $m'+m=l$, be the individual subassemblies remaining on the path, in order, so that $P=(P'(1), \ldots, P'(m'),\beta_1,\ldots,\beta_m)$.
  For all $1 \leq i \leq m$, let $\gamma_i = \bigcup_{j=1}^i \beta_j$ be the next $i$ such subassemblies on the path.
  Let $s_i = |\gamma_i|$ be the size of the $i^\text{th}$ subassembly, and let $c_i(t) = \sum_{\alpha' \in A_i(t)} [\alpha'](t)$, where $A_i(t)$ is the set of subassemblies (possibly containing tiles not on the path $P$) at time $t_0$ that contain $\gamma_i$ but do not contain $\gamma_{i+1}$.
  For each $1 \leq i \leq m$, in the next instant $dt$, with probability $c_i dt$ the prefix will extend by total weighted length $s_i$ by attachment of (a superassembly containing) $\gamma_i$.
  This implies that $f'(t) \leq \sum_{i=1}^m c_i(t) \cdot s_i$.
  Invoking Lemma~\ref{lem-constant-sum-conc}, it follows that for all $t\in\R^+$,
  \[
    f'(t)
    \leq
    \sum_{i=1}^m c_i(t) \cdot s_i
    \leq
    \sum_{\alpha \in \prodasm{\calT}} [\alpha](t) \cdot |\alpha|
    =
    1. \qedhere
  \]
}

\opt{normal}{
    \begin{proof}
    \ProofHierPartialOrderSlow
    \end{proof}
}






==> two-handed-square.tex <==
\section{Hierarchical Self-Assembly: Parallelism and Time}
\label{sec-hierarchical}


\opt{normal}{
%The results of this section concern only the hierarchical aTAM.
In this section we show that under the hierarchical model of tile assembly, it is possible to self-assemble an $n \times n$ square, for arbitrary $n \in \Z^+$, using the asymptotically optimal $O(\frac{\log n}{\log \log n})$ number of tile types.
Furthermore, the square assembles using nearly the maximum possible parallelism in the hierarchical model, building the final square out of four assembled sub-squares of size $n/2 \times n/2$, which are themselves each assembled from four sub-squares of size $n/4 \times n/4$, etc.
(The sub-optimality stems from the need for us to construct the smallest sub-squares of size $O(\log n) \times O(\log n) = O(\log^2 n)$ without parallelism.)

We then show that, somewhat counterintuitively, this construction is \emph{slower} than the construction of~\cite{AdChGoHu01}, which assembles an $n \times n$ square in time $O(n)$ in the seeded aTAM. %in which tiles are only permitted to attach to the seed assembly one at a time.
The authors of \cite{AdChGoHu01} define a class of seeded TAS's called \emph{partial order systems}, whose definition we extend in a natural way to hierarchical systems.
We show, using basic principles of chemical kinetics, that \emph{no} partial order system can assemble any shape of size $N$ in faster than $\Omega(\sqrt{N})$ time.
Thus hierarchical partial order systems achieve no speedup at all over seeded systems.
%This implies that among partial order systems, the TAS described in~\cite{AdChGoHu01} for assembling an $n \times n$ square is in fact optimal, in both tile complexity and in assembly time, for the hierarchical model as well.
%We note, however, that there are other theoretical advantages to the hierarchical model, for instance, the use of steric hindrance to enable algorithmic fault-tolerance~\cite{DotPatReiSchSum10}.
}



\subsection{Nearly Maximally Parallel Hierarchical Assembly of an $n \times n$ Square with Optimal Tile Complexity}
\label{sec-hierarchical-square}

\opt{normal}{
We formalize the notion of ``parallelism through hierarchical assembly'' as follows.
}

\opt{submission}{
We give a formal definition of ``parallelism through hierarchical assembly'' in Section~\ref{sec-app-parallel-square}, which defines $\Kddac(\calT)$ as the maximum depth of any ``assembly tree'' of $\calT$.
}

\newcommand{\ParallelDefn}{
    Let $\calT=(T,g,\tau)$ be a directed hierarchical TAS.
    Let $\alpha \in \prodasm{\calT}$ be a producible assembly.
    An \emph{assembly tree} $\Upsilon$ of $\alpha$ is a binary tree whose nodes are labeled by producible assemblies, with $\alpha$ labeling the root, individual tile types labeling the $|\dom \alpha|$ leaves, and node $u$ having children $u_1$ and $u_2$ with the requirement that $u_1$ and $u_2$ can attach to assemble $v$.
    That is, $\Upsilon$ represents one possible pathway through which $\alpha$ could be produced from individual tile types in $\calT$.
    Let $\Upsilon(\calT)$ denote the set of all assembly trees of $\calT$.
    Say that an assembly tree is \emph{terminal} if its root is a terminal assembly.
    %An assembly can be terminal even if T is not directed, so we can define a terminal assembly tree for any TAS, not just terminal systems.
    Let $\Upsilon_\Box(\calT)$ denote the set of all terminal assembly trees of $\calT$.
    Note that even a directed hierarchical TAS can have multiple terminal assembly trees that all have the same root terminal assembly.
    The \emph{assembly depth} of $\calT$ is
    $
        \Kddac(\calT) = \max_{A \in \Upsilon_\Box(\calT)} \mathrm{depth}(A),
    $
    where $\mathrm{depth}(A)$ denotes the standard depth of the tree $A$, the length of the longest path from any leaf to the root.
    Let $S \subset \Z^2$ be a finite shape.
    The \emph{directed assembly depth} of $S$ is
    $$\Kddac(S) = \min \setr{\Kddac(\calT)}{\begin{array}{l}
    \calT=(T,g,\tau) \text{ is a directed hierarchical}
     \\
     \text{TAS and } \calT \text{ strictly self-assembles } S
     \end{array}}.$$


     It is clear by the definition that for any shape $S$ with $N$ points, $\Kddac(S) \geq \log N$.
     Our construction nearly achieves this bound in the case of assembling an $n \times n$ square $S_n$, showing that $\Kddac(S_n) \leq O(\log^2 n)$.
     In other words, not only is it the case that every producible assembly can assemble into the terminal assembly (by the definition of directed), but in fact every producible assembly is at most $O(\log^2 n)$ attachment events from becoming the terminal assembly.

     Furthermore, we achieve nearly optimal tile complexity in additional to optimal assembly depth.
     In~\cite{AGKS05}, the authors prove that whenever $n \in \N$ is algorithmically random, at least $\Omega(\log n / \log \log n)$ tile types are required to strictly self-assemble an $n \times n$ square in the hierarchical model.
     Actually, that paper states only that this holds for the \emph{$q$-tile model}, in which some constant $q$ exists that limits the size of attachable assemblies other than those containing a special seed tile, and the authors claim that the proof requires the bound $q$, but in fact their proof does not use the bound $q$ and works for the general hierarchical model~\cite{RobbiePersonal2010}.
}

\opt{normal}{\ParallelDefn}









\newcommand{\FigSquareHighLevelCaption}{
  Overview of the hierarchical TAS that assembles an $n \times n$ square with $O(\log^2 n)$ assembly depth and $O(\frac{\log n}{\log \log n})$ tile complexity.
  Each square in the figure represents a block of width $O(\log n)$ with the all sides of each block encoding its $(x,y)$-address in the square.
  \opt{normal}{(The encoding scheme is shown in more detail in Figure~\ref{fig:two-handed-square-block}.)}
  Each of the thin solid lines is a strength-1 glue; in fact they are all identical.
  Dotted lines connect those glues that are intended to bind to each other.
  The circled subassemblies show the order of growth of one particular block (at coordinates $(3,2)$) into the final square.
}

\opt{normal}{
    \begin{figure}[htb]
    \begin{center}
      \includegraphics[width=5.7in]{figures/two-handed-square-high-level}
      \caption{\label{fig:two-handed-square-high-level} \figuresize
      \FigSquareHighLevelCaption
      }
    \end{center}
    \end{figure}
}



\newcommand{\FigNonPowTwo}{
    \begin{figure}[htb]
    \begin{center}
      \includegraphics[width=4in]{figures/two-handed-square-non-power-of-2}
      \caption{\label{fig:two-handed-square-non-power-of-2} \figuresize
      Design of block sizes to handle values of $n$ that are not a power of two. There are always exactly $2^k \times 2^k$ blocks, where $2^k \leq n < 2^{k+1}$.
      Each block doubles the length of its along the $x$-axis (resp. $y$-axis) if $n - 2^k$ exceeds its $x$-coordinate (resp. $y$-coordinate).
      The solid lines represent block boundaries, and the dotted lines are to help visualize the size of the square.}
    \end{center}
    \end{figure}
}


\newcommand{\FigBlock}{
    \begin{figure}[htb]
    \begin{center}
      \includegraphics[width=6.5in]{figures/two-handed-square-block}
      \caption{\label{fig:two-handed-square-block} \figuresize
      Assembly of $O(\log n) \times O(\log n)$ size block from $O(\frac{\log n}{\log \log n})$ tile types.
      Every block starts from the same tile types that encode $n-2^k$, using exactly $k$ bits; in this example, $n=22$ so $k=4$ and $n-2^k$ is 0110 in binary using 4 bits.
      Thick solid lines represent strength-2 glues.
      For clarity, strength-1 glues are shown selectively to help verify that a certain order of growth is possible to enforce.
      The tiles encode $n-2^k$ in base $b$ chosen to be a power of two such that $\frac{\log n}{\log \log n} \leq b < 2  \frac{\log n}{\log \log n}$ (labeled ``seed'' for intuition, although those tiles start unattached).
      A constant-size set of tile types does the rest.
      $n-2^k$ is first converted to binary and each of its bits quadrupled to make room for the bumps and dents.
      Then $x$ and $y$ coordinates are randomly guessed and simultaneously compared to $n-2^k$; if either is smaller, that dimension is doubled in length (in this example the height is doubled but not the width).
      At the same time, the values of $x$ and $y$ are compared as described in the proof of Theorem~\ref{thm-hierarchical-square} to determine where to place strength-1 glues.}
    \end{center}
    \end{figure}
}

\opt{normal}{
    \FigNonPowTwo

    \FigBlock
}


 \begin{theorem} \label{thm-hierarchical-square}
   There are constants $c_1,c_2\in\N$ such that, for all $n\in\N$, there is a directed hierarchical TAS $\calT=(T,g,2)$ such that $\calT$ strictly self-assembles the $n \times n$ square, $|T| \leq c_1 \log n / \log \log n$, and $\Kddac(\calT) \leq c_2 \log^2 n$.
 \end{theorem}

\opt{submission}{
    A formal proof of Theorem~\ref{thm-hierarchical-square} is contained in Section~\ref{sec-app-parallel-square}.
    Figure~\ref{fig:two-handed-square-high-level} shows the high-level idea.
    The figure shows how to create a square of $n \times n$ blocks, each of width $O(\log n)$, for $n$ a power of two.
    The full proof explains how to handle $n$ that are not a power of two and how to handle $n$ that are not perfectly divisible by the block length.
    Intuitively, tiles aggregate into blocks while randomly guessing their ``$(x,y)$ address'' in the final square.
    The blocks encode this address into the bumps and dents on the side of the block, which ensures that fully formed blocks can only bind to their neighbors (the strength-1 glues shown in Figure~\ref{fig:two-handed-square-high-level} are all identical so the bumps and dents are required to encode this specificity.)
    The growth order of the blocks enforces that the strength-1 glues needed for binding are not present until enough bumps and dents are present to enforce this binding specificity.
    The $(x,y)$ address is also used to determine where to put strength-1 glues, since not all sides of all blocks have them.
    This enforces the ``recursive doubling'' of Figure~\ref{fig:two-handed-square-high-level}, namely that all blocks bind without overlap, so that blocks at level $i$ of the recursive hierarchy cannot bind to their level $i$ ``twin'' set of blocks until both have completely finished all level $i-1$ binding.
}


\newcommand{\ProofParallelSquare}{
   A high-level outline of the construction is shown in Figure~\ref{fig:two-handed-square-high-level}.
   We assemble a number of blocks of width $O(\log n) \times O(\log n)$, each of which represents in its tile types an address indicating its position in the square, and the block binds only to (some of) its neighboring blocks.
   The blocks assemble using standard single-tile accretion (actually we cannot directly enforce this in the model, but each block will nonetheless assemble the same structure in either model).
   Since each block is $O(\log^2 n)$ total tiles, this is the source of the suboptimal $O(\log^2 n)$ assembly depth.
   Once the blocks are assembled, however, they assemble into the full square using $O(\log n)$ assembly depth.
   All blocks $(x,y)$ with $x$ even bind to $(x+1)$ to create the two-block assembly $(x,y):(x+1,y)$, then all blocks $(x,y):(x+1,y)$ with $y$ even bind to $(x,y+1):(x+1,y+1)$ to create the four-block assembly $(x,y):(x+1,y):(x,y+1):(x+1,y+1)$, etc.


   The construction will actually control the width of the square only to within an additive logarithmic factor by bring together blocks of width and length $\Theta(\log n)$; standard techniques can be used to make the square precisely $n \times n$.
   For instance, we could add $O(\log n)$ total filler tiles to the leftmost and bottommost blocks, while adding only $O(\log^2 n)$ to the assembly depth and $O(\log \log n)$ to the tile complexity since such filler tiles could be assembled from a counter that counts to $\log n$ using $O(\log \log n)$ tile types.
   For simplicity we describe the desired width $n$ as the number of blocks instead of the desired dimensions of the square and omit the details of this last step of filling in the logarithmic gap.

   Figure~\ref{fig:two-handed-square-high-level} outlines the construction of a square when the number of blocks $n$ is a power of two.
   Figure~\ref{fig:two-handed-square-non-power-of-2} shows how to modify the blocks so that some of them are double in width, double in height, or both, to achieve a total square width that is an arbitrary positive integer.
   Each block contains the same $O(\frac{\log n}{\log \log n})$ tile types that encode $n$, and as the block assembles it randomly chooses $x$ and $y$-coordinates, which represent an index in the square.
   This random choice is implemented through competition between tile types that share the same ``input'' glues but represent different bits of $x$ or $y$.%\footnote{A curious feature of hierarchical TAS's is that the TAS can remain directed despite this nondeterministic competition, whereas it cannot happen in any directed seeded TAS.}
   These are used to determine the block's own size and to determine what series of bumps and dents to place on its perimeter to enforce that the only blocks that can bind are adjacent in Figure~\ref{fig:two-handed-square-high-level}.
   The coordinates are also used to determine where to place strength-1 glues. The same strength-1 glue is used uniformly throughout Figure~\ref{fig:two-handed-square-high-level}.
   The bumps and dents ensure that no two blocks can attach unless they are adjacent in the figure.

   The growth of an individual block is shown in Figure~\ref{fig:two-handed-square-block}.
   We describe the assembly as if it grows only by single-tile accretion.
   There are some strength-2 glues so this is not completely accurate, but the growth of the block is ``polyomino-safe'', to borrow a term of Winfree~\cite{Winfree06}.
   By design, no assembly larger than four can form except by attachment to the growing block, and even if these assemblies attach at once to the block rather than by single-tile accretion, the correct operation of the block growth is unaffected.
   This is due to the fact that all strength-2 glues are ``position-unique''; no strength-2 glue is shared between two points in Figure~\ref{fig:two-handed-square-block}, and by inspection no partial assembly occurring away from the main ``seeded'' assembly can grow ``backward'' and place an incorrect tile.

   To form a square of size $n \times n$ ``units'' (where a unit is $O(\log n)$, the width and height of a small block), we choose the largest power of two $2^k \leq n$ and assemble exactly $2^k \times 2^k$ different types of blocks, doubling the width (resp. height) of the first $n-2^k$ of them in the $x$-direction (resp. $y$-direction), as in Figure~\ref{fig:two-handed-square-non-power-of-2}.
   The orange (medium darkness in gray-scale) tile types in Figure~\ref{fig:two-handed-square-block} are the only non-constant set of tile types.
   Borrowing a technique from~\cite{AdChGoHu01}, we will represent $n$ in base $b$, where $b \approx \log n / \log \log n$, using $\approx \log n / \log \log n$ unique tile types, and we use a constant number of tile types to convert $n-2^k$ to binary and accomplish all the other tasks needed to assemble the block.

   Choose $b=2^m$ to be a power of two such that $\log n / \log \log n \leq b < 2 \log n / \log \log n.$
   Each digit in base $b$ can represent $m$ bits of $n-2^k$.
   $n-2^k$ is encoded in exactly $m \cdot \ceil{\frac{k}{m}} = O(\frac{\log n}{\log \log n})$ base-$b$ digits.
   The blue (dark in gray-scale) tile types in Figure~\ref{fig:two-handed-square-block} convert $n-2^k$ from base $b$ to binary and at the same time represent $n-2^k$ with its ``bit-quadrupled'' version (e.g., $0110 \mapsto 0000111111110000$), since each bit along the edge will eventually require width four to make room to place the bumps properly.\footnote{The bumps cannot simply be placed with strength-2 glues above a width-1 or even width-2 representation of a bit in the obvious way, otherwise there would be nothing to force that the bumps are present before the inter-block strength-1 glues.  If the bumps are allowed to grow in parallel with the rest of the assembly then they may not complete fast enough.  Width four is required to create a ``linear assembly path'' for the bumps and dents tiles to follow, ensuring that growth of the block continues only once the path is complete.}
   %At the same time $n-2^k$ is converted to binary, every fourth position along the row, there is a nondeterministic competition among four tile types to determine a bit of $x$ and a bit of $y$.
   The counterclockwise order of growth ensures that if not all of the bumps and dents are formed, then at least one of the four strength-1 glues necessary for an attachment event to occur is not yet present in one of the blocks.
   To ensure that the TAS is directed, we do not include base-conversion tiles for any digit $d \in \{0,1,\ldots,b-1\}$ that does not appear in the base-$b$ expansion of $n-2^k$, otherwise those tiles will form unused terminal assemblies.
   Each glue in a tile type representing a bit is ``marked'' indicating whether it is the most significant bit, least significant bit, or interior bit, as well as being marked with its relative position among the four copies of the bit.

   Once $n-2^k$ is converted to binary, we use nondeterministic attachment of tiles to the north of this value to randomly guess $2k$ bits that represent the $x$- and $y$-coordinates of the block, meaning the binary numbers represented on the top and right, respectively, of each block in Figure~\ref{fig:two-handed-square-high-level}.
   To be precise, we must actually choose each of $x$ and $y$ to be a random bit string that is not all 1's, since each represents a connection between two blocks, of which there are $2^k-1$ along each dimension.
   It is straightforward to encode into the tile types the logic that if the first $k$ bits were 1, then the final bit must be 0.
   A number of additional computations are done on these values (some computations are possible to do as the values are guessed).
   The results of these computations will be stored in the rightmost tile type and propagated to all subsequent tile types.
   First, each of $x$ and $y$ is compared to $n-2^k$ to determine how large to make each dimension of the block.
   In the example of Figure~\ref{fig:two-handed-square-block}, $y < n-2^k$ and $x \geq n-2^k$, so the block is one ``unit'' wide and two ``units'' high.
   Also, the binary expansions of $x$ and $y$ are themselves compared to determine where to place strength-1 glues.
   After $x$ and $y$ are determined, to place bumps and dents on the left and bottom of the block, the values $x-1$ and $y-1$ must be computed, which requires assembling from least significant to most significant, so this is delayed until after the first 90-degree rotation shown in Figure~\ref{fig:two-handed-square-block}.
   Once these values are computed, they are also used to determine placement of glues.
   The entire block is created by rotating either counter-clockwise (in the case of $x$ even, as shown in the bottom right of Figure~\ref{fig:two-handed-square-block}) or clockwise (in the case of $x$ odd, not shown but the exact mirror image of the bottom right of Figure~\ref{fig:two-handed-square-block}), placing bumps and dents and single-strength glues.
   The glues are placed in the order shown by the rotations, so that the last glue to be (potentially) placed is the top east-facing glue in the case of $x$ even, or the top west-facing glue in the case of $x$ odd.


   By inspection of Figure~\ref{fig:two-handed-square-high-level}, it is routine to verify that the following rules can be used to determine placement of strength-1 glues.
   If $x$ is even, then place two single-strength glues on the right edge.
   If $x$ is odd, then place two single-strength glues on the left edge.
   For a natural number $n$, define $t(n)$ to be the number of trailing 1's in $n$'s binary expansion.
   If $t(x) \geq t(y)$, then place exactly one strength-1 glue on the top edge.
   If $t(x) \geq t(y-1)$, then place exactly one strength-1 glue on the bottom edge.
   If $t(x-1) \leq t(y)+1$ and $x$ is even, then place exactly one strength-1 glue on the left edge.
   If $t(x) \leq t(y)+1$ and $x$ is odd, then place exactly one strength-1 glue on the right edge.

   Each of these computations (for placement of glues and for determining block dimensions) can be computed by a deterministic finite automaton whose input symbols represent tuples of bits from $n-2^k$, $x$, $x-1$, $y-1$, and $y$.
   These automata can then be combined in a product construction and embedded into the tile types that accrete in the row above $n-2^k$ if only $x$ and $y$ are needed, and embedded into tile types that are placed after the first rotation if $x-1$ or $y-1$ is needed.
   Since the decision for placing glue on the top edge requires only $x$ and $y$, this ensures that the decision for each glue placement can be made before the region containing the potential glue site is assembled.

   As shown in Figure~\ref{fig:two-handed-square-block}, some padding with filler tiles is necessary to make the block a perfect rectangle.
   Also, some padding is needed in the case of a doubling of height or width, to ensure that the resulting assembly has height or width precisely twice that of the non-doubled version.
}

\opt{normal}{
    \begin{proof}
    \ProofParallelSquare
    \end{proof}
}



















\subsection{Time Complexity in the Hierarchical Model}
\label{sec-runtime}





\input{two-handed-assembly-time}


